Sequential data assimilation with multiple nonlinear models and applications to subsurface flow

Complex systems are often described with competing models. Such divergence of interpretation on the system may stem from model fidelity, mathematical simplicity, and more generally, our limited knowledge of the underlying processes. Meanwhile, available but limited observations of system state could further complicates one's prediction choices. Over the years, data assimilation techniques, such as the Kalman filter, have become essential tools for improved system estimation by incorporating both models forecast and measurement; but its potential to mitigate the impacts of aforementioned model-form uncertainty has yet to be developed. Based on an earlier study of Multi-model Kalman filter, we propose a novel framework to assimilate multiple models with observation data for nonlinear systems, using extended Kalman filter, ensemble Kalman filter and particle filter, respectively. Through numerical examples of subsurface flow, we demonstrate that the new assimilation framework provides an effective and improved forecast of system behaviour.

==> Sections/Examples/hetero.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multi-model assimilations for heterogeneous soil}
\label{sec:exs-heter}

Now we introduce soil heterogeneity to the flow domain and illustrate the effectiveness of our DA framework on quantifying both model-form and parametric uncertainty.  To be specific, we adopt the statistical settings of earlier works~\cite{wang-2011-reduced} and treat the saturated hydraulic conductivity and van Genuchen parameter as mutually-uncorrelated log-normal random fields, e.g., $ln K_s(\mathbf x) \sim \mathcal N(-3.58, 0.89)$ and $ln \alpha(\mathbf x) \sim \mathcal N(-3.01, 0.63)$, respectively. Using the geo-statistical library SGEMS, a total of $2000$ realizations are generated for $K_s(\mathbf x) $ and $\alpha(\mathbf x) $ in a two-dimensional ($15,000 \times 200 \, cm^2)$ domain discretized into $2500$ nodes.  We prescribe an anisotropic exponential correlation function for both parameter. To satisfy the Dagan-Bresler parameterization~\cite{dagan-1983-unsaturated}, the vertical and horizontal correlation lengths ratio are set as $\lambda_v / \lambda_h = 18.75$ and $30.0$ for the random fields $\ln K_s$ and $\ln \alpha$, respectively. 

For each realization of $K_s(\mathbf x)$ and $\alpha(\mathbf x)$, we solve the Richards equation with VS2DT and determine the infiltration rate $i(t)$ at a surface midpoint. The results were used to compute the ``true" infiltration-rate PDF as 
%
\begin{equation} \label{eqn:MCS}
	p_{\mathrm i}(i^\star;t)= \frac{1}{2000 \Delta_{bin}} \sum_{n=1}^{2000} I(i_n \in \Delta_{bin}^{i^\star};t), 
\eng{equation
%
where $\Delta_{bin}$ is a (uniform) bin size, $\Delta_{bin}^{i^\star}$ is the bin containing $i^\star$, and $I$ is the indicator function. We select an equi-spaced entries within the {\it mean} Richards solution vector, $\langle i (t) \rangle = \sum_{n=1}^{2000} i_n(t)/2000$, and add a fluctuation $\e_d \sim \mathcal N (0,0.002^2)$. This is our noisy observation data and would be assimilated using particle filter (PF) scheme, with an array of $1000$ forecasts from Green-Ampt and Parlange models, respectively. We note here that Dagan-Bresler parameterization~\cite{dagan-1983-unsaturated} allows us to replace the random fields as random constants: $ln K_s(\mathbf x) \sim ln K_s$ and $ln \alpha(\mathbf x) \sim ln \alpha$. Hence samples of $K_s$ and $\alpha$ can be used to obtain $p_{\mathrm i}$ using the two reduced-complexity models, separately~\cite{wang-2011-probabilistic, wang-2011-reduced}. 

Figure~\ref{fig:pf-MCS} presents the infiltration rate PDF $p_{\mathrm i}(i^\star;t=5 \, min)$, computed from the forecasts of Green-Ampt model, Parlange model, their multi-model PF scheme \annote{line} and the MCS results from VS2DT. Here our observation data is shown as a column of circles and the reference model of PF scheme is \annote{Green-Ampt/Parlange}.

From Fig.~\ref{fig:pf-MCS}, it is clear that the multi-model assimilation yields a distribution with narrower width, an indication of less uncertain (e.g. more accurate) prediction than that of any single model.

%
\begin{figure}[htbp]
\begin{center}
\includegraphics[width=8in]{Figures/figure_pdf_particle_filter_5min} 
%\includegraphics[width=4in]{Figures/figure_pdf_particle_filter_10min} 
\caption{The infiltration rate PDF $p_{\mathrm i}(i^\star;t=5 \, min)$ computed from the forecasts of Green-Ampt model (Dash-dot line), Parlange model (dashed line), their multi-model particle filter scheme \annote{line} and the MCS results from VS2DT (dotted line). Here the observation data is shown as a column of circles and the reference model of PF scheme is \annote{Green-Ampt/Parlange}.} 
\label{fig:pf-MCS} 
\end{center}
\end{figure}
%


